AFN: Adaptive Fusion Normalization via an Encoder-Decoder Framework

The success of deep learning is inseparable from normalization layers. Researchers have proposed various normalization functions, and each of them has both advantages and disadvantages. In response, efforts have been made to design a unified normalization function that combines all normalization procedures and mitigates their weaknesses. We also proposed a new normalization function called Adaptive Fusion Normalization. Through experiments, we demonstrate AFN outperforms the previous normalization techniques in domain generalization and image classification tasks.

==> sections/normalization.tex <==
% intro part
In the past decades, researchers made great progress on deep learning, and applied deep learning in many fields, including computer vision, natural language processing, speech, and reinforcement learning. Deep learning has achieved remarkable success in various areas, where the training and test data are in the same domain~\cite{LeCun2015DeepL, Krizhevsky2012ImageNetCW, shao2022learning}. However, in real applications, it is common to apply a deep learning model to the data from a new domain unseen in the training dataset. The model that performs well on the training domain usually cannot maintain a consistent performance on a new domain, due to the cross-domain distributional shift~\cite{Nado2020EvaluatingPB}. In order to solve this problem, researchers have proposed manifold normalisation methods~\cite{BatchNorm, GroupNorm, SwitchNorm, LayerNorm, Ulyanov2016InstanceNT}.
%





%
The previous normalisation methods follow the same formula, but the mean and variance are derived in  different ways:
\begin{center}
    \begin{align}
            y =  \gamma * \frac{(x - \mu)}{\sigma+\epsilon} + \beta, 
    \end{align}
\end{center}
where $\gamma$, $\beta$ are learnable parameters, and $\epsilon$ is a very small number to prevent mathmatical errors.



\subsection{Batch Normalisation}
In 2015, Ioffe and Szegedy proposed Batch Normalisation\~cite{BatchNorm} to better accelerate deep network training and reduce the internal covariate shift.
Given an input mini-batch, the method will normalise the feature map through a specific feature channel of all data to reach better performance.
For an input feature map with shape $(N,C,H,D)$, where $N$ is the batch size, $C$ is the number of channels, and $H$, $D$ are the width and high of the feature map, respectively.
Batch Normalisation performs as:

\begin{center}
\begin{align}
    \mu = \sum_{i=1}^{N*H*D} x_i / (N*H*D)  \\
    \sigma =\sqrt{ \sum_{i=1}^{N*H*D} (x_i-\mu)^2 / (N*H*D)}.
\end{align}
\end{center}


\subsection{Layer Normalisation}
 From the methodology of batch normalisation, it needs a big batch size to reasonably get the mean and variance of data, which leads to great use of memory. Without enough batch size, batch normalisation performs badly. Also, batch normalisation is difficult to apply for RNN models. Layer Normalzation~\cite{LayerNorm} is proposed to solve these problems. It holds the same formula as batch normalisation, but layer normalisation computes the mean and variance from all features of all channels in one specific data.
 \begin{align}
    \mu = \sum_{i=1}^{C*H*D} x_i / (C*H*D)  \\
    \sigma =\sqrt{ \sum_{i=1}^{C*H*D} (x_i-\mu)^2 / (C*H*D)}
 \end{align}
    where H denotes the number of hidden units in a layer.

 \subsection{Instance Normalisation}
 In the image style transfer task, the mean and variance of each channel of the feature map, which is calculated by the generative model will influence the style of the generated image. So researchers put forward the Instance Normalisation~\cite{Ulyanov2016InstanceNT}.
Instance Normalisation computes the mean and variate from (H,W) dimension on a specific channel of a specific data.
\begin{align}
    \mu = \sum_{i=1}^{H*D} x_i / (H*D)  \\
    \sigma =\sqrt{ \sum_{i=1}^{H*D} (x_i-\mu)^2 / (H*D)}
\end{align}

\subsection{Group Normalisation}
As mentioned before, batch normalisation has a bad performance when the batch size gets smaller and smaller. In order to solve this problem, a new method, called group normalisation~\cite{GroupNorm} is proposed. Group normalisation divides channels into different groups, and for each group, it applies normalisation like instance normalisation.
\begin{align}
    \mu = \frac{1}{m}\sum_{k\in{S_i}}x_k \\ 
    \sigma = \sqrt{\frac{1}{m}\sum_{k\in{S_i}}(x_k-\mu_i)^2+\epsilon}
\end{align}
$\epsilon$ is a small constant. $S_i$ is the set of pixels in which the mean and std are computed, and $m$ is the size of this set.

% BIN formula
\begin{align}
    y = (\rho \cdot \hat{x}^{(B)} + (1 - \rho) \cdot \hat{x}^{(I)}) \cdot \gamma + \beta
\end{align}
where the $\hat{x}^{(B)}$ is the batch-normalised response, and the $\hat{x}^{(I)}$ is the instance-normalised response. $\rho$ is the additional learnable parameters range in [0, 1], imposing bounds at the parameter update step.
\begin{align}
    \rho \xleftarrow{}clip_{[0,1]}(\rho - \eta\Delta\rho)
\end{align}
$\gamma$ and $\beta \in R^C$ are the affine transformation parameters and $y$ $\in R^{N \times C \times H \times W}$ is the output of BIN.
